Deformable 3D Shape Diffusion Model

The Gaussian diffusion model, initially designed for image generation, has recently been adapted for 3D point cloud generation. However, these adaptations have not fully considered the intrinsic geometric characteristics of 3D shapes, thereby constraining the diffusion model's potential for 3D shape manipulation. To address this limitation, we introduce a novel deformable 3D shape diffusion model that facilitates comprehensive 3D shape manipulation, including point cloud generation, mesh deformation, and facial animation. Our approach innovatively incorporates a differential deformation kernel, which deconstructs the generation of geometric structures into successive non-rigid deformation stages. By leveraging a probabilistic diffusion model to simulate this step-by-step process, our method provides a versatile and efficient solution for a wide range of applications, spanning from graphics rendering to facial expression animation. Empirical evidence highlights the effectiveness of our approach, demonstrating state-of-the-art performance in point cloud generation and competitive results in mesh deformation. Additionally, extensive visual demonstrations reveal the significant potential of our approach for practical applications. Our method presents a unique pathway for advancing 3D shape manipulation and unlocking new opportunities in the realm of virtual reality.

==> fig/tex/backbone.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/pdf/backbone.pdf}
    \caption{Illustration of a PointNet++ backbone integrated with transformer blocks.}
    \label{fig: backbone}
\end{figure}

==> fig/tex/face.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/pdf/face_aggresive.pdf}
    \caption{
    Progressive animation of facial expression.
    $\mathcal{X}^{(9)}$ is the initial face without any expression.
    The first row shows the originally generated facial meshes.
    The differences between two consecutive facial meshes are highlighted in the second row for easier comparison. 
    }
    \label{fig: face}
\end{figure*}

==> fig/tex/face_mesh.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/pdf/face_mesh.pdf}
    \caption{
    The mesh structure of the generated face.
    The mesh on the left is the template shape $\mathcal{X}^{(T)}$, and the one on the right is the generated face $\mathcal{X}^{(0)}$.
    }
    \label{fig: face mesh}
\end{figure}

==> fig/tex/progressive_mesh_generation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/pdf/progressive_generation_mesh.pdf}
    \caption{The process of progressively generating meshes.}
    \label{fig: progressive mesh generation}
\end{figure}

==> fig/tex/progressive_pcl_generation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/pdf/progressive_generation_pcl.pdf}
    \caption{The process of progressively generating point clouds.}
    \label{fig: progressive pcl generation}
\end{figure}

==> tab/network.tex <==
\begin{table}[htb]
\caption{Data flow.}
\label{tab. data flow}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|c}
layer               & input                         & output                & embedding dims \\ \hline
time embedding      & \textbf{timesteps}            & time emb.             & $d_{time}$     \\
initial projection  & \textbf{points}               & $l_0$ feat.           & 64             \\ \hline
time scale shift    & $l_0$ feat., time emb.        & $l_0$ emb.            & 64             \\
set abstraction msg & $l_0$ emb.                    & $l_1$ feat.           & 320            \\
time scale shift    & $l_1$ feat., time emb.        & $l_1$ emb.            & 320            \\
set abstraction msg & $l_1$ emb.                    & $l_2$ feat.           & 512            \\
time scale shift    & $l_2$ feat., time emb.        & $l_2$ emb.            & 512            \\
set abstraction     & $l_2$ emb.                    & $l_3$ feat.           & 1024           \\
time scale shift    & $l_3$ feat., time emb.        & $l_3$ emb.            & 1024           \\
feature propagation & $l_2$ emb., $l_3$ emb.        & $l_2^\prime$ feat.    & 256            \\
time scale shift    & $l_2^\prime$ feat., time emb. & $l_{2}^\prime$ emb.   & 256            \\
feature propagation & $l_1$ emb., $l_2^\prime$ emb. & $l_1^\prime$ feat.    & 128            \\
time scale shift    & $l_1^\prime$ feat., time emb. & $l_{1}^\prime$ emb.   & 128            \\
feature propagation & $l_0$ emb., $l_1^\prime$ emb. & $l_0^\prime$ feat.    & 128            \\
time scale shift    & $l_0^\prime$ feat., time emb. & $l_0^\prime$ emb.     & 128            \\
mlp layers          & $l_0^\prime$ emb.             & offset                & 3              \\ \hline
scale layer         & offset                        & \textbf{scaled offet} & 3             
\end{tabular}
}
\end{table}
